NeBula: Quest for Robotic Autonomy in Challenging Environments; TEAM CoSTAR at the DARPA Subterranean Challenge

This paper presents and discusses algorithms, hardware, and software architecture developed by the TEAM CoSTAR (Collaborative SubTerranean Autonomous Robots), competing in the DARPA Subterranean Challenge. Specifically, it presents the techniques utilized within the Tunnel (2019) and Urban (2020) competitions, where CoSTAR achieved 2nd and 1st place, respectively. We also discuss CoSTAR's demonstrations in Martian-analog surface and subsurface (lava tubes) exploration. The paper introduces our autonomy solution, referred to as NeBula (Networked Belief-aware Perceptual Autonomy). NeBula is an uncertainty-aware framework that aims at enabling resilient and modular autonomy solutions by performing reasoning and decision making in the belief space (space of probability distributions over the robot and world states). We discuss various components of the NeBula framework, including: (i) geometric and semantic environment mapping; (ii) a multi-modal positioning system; (iii) traversability analysis and local planning; (iv) global motion planning and exploration behavior; (i) risk-aware mission planning; (vi) networking and decentralized reasoning; and (vii) learning-enabled adaptation. We discuss the performance of NeBula on several robot types (e.g. wheeled, legged, flying), in various environments. We discuss the specific results and lessons learned from fielding this solution in the challenging courses of the DARPA Subterranean Challenge competition.

==> sections/5.Delete_state_estimation.tex <==
% This file is NOT being used
% This file is NOT being used
% This file is NOT being used
% This file is NOT being used
% This file is NOT being used
% This file is NOT being used
% This file is NOT being used
\section{State Estimation \comb{Angel}}

A reliable and robust state estimation is one of the fundamental components of NeBula (See \autoref{?nebula-arch?}). In particular, NeBula focuses on developing estimators and odometry methods that are resilient under perceptually-degraded conditions, including variable lighting, obscurants (dust, fog, smoke), full dark, feature-less or self-similar environment, among others. In this section, we briefly go over NeBula's state estimation module. For more details, see \cite{hero, seyedOld, seyedNew, ...}

\ph{Related work focuses on accuracy and not robustness}
The main body of literature in robot state estimation focuses on developing complex algorithms favoring accuracy and leaving the overall robustness still as an open challenge.
Typically, these methods possess a single point of failure: the main estimation engine is assumed not to fail during operation; and are not able to recover upon breakdown, leading to catastrophic failures in the navigation stack.
This is the case of approaches which combine data from several sensors into one tightly coupled estimation engine, \emph{e.g.}, \cite{Zhang2015ICRA,Tomic2012AutonUAV,weissmonocular,Santamaria-NavarroAuro18}.
For example, KITTI dataset \cite{Geiger2012CVPR} benchmarks accuracy of more than 100 approaches that fuse visual information (monocular, stereo or RGB-D cameras), range measurements (SoNAR or LiDAR) and inertial measurements (IMU). 
Heterogeneity and redundancy of sensors has been exploited to partially achieve estimation robustness in methods like \cite{rollinson2013robust,nobili2017heterogeneous,Gosala2018RedundantPA,Carnevaleijars2015,kim2019resiliency} for legged, snake-like and race car robots, respectively.
However, these architectures still rely on a single estimation engine.

\ph{Describe how our algorithm overcomes the above}
To pursue robustness in state estimation we propose an architecture, shown in Figure~\ref{fig:hero}, which considers redundancy and heterogeneity in both sensing and estimation algorithms, and it is designed to expect and detect failures while adapting the behavior of the system to ensure safety.
To this end, we present HeRO (Heterogeneous Resilient Odometry): a stack of estimation algorithms running in parallel supervised by a resiliency logic.
This logic carries out three main functions: a) Perform confidence tests both in data quality (measurements and individual estimations) and check health of sensors and algorithms; b) Re-initialize those algorithms that might be malfunctioning; c) Generate a smooth state estimate by multiplexing the inputs based on their quality.
The output of this resiliency logic is fed into the guidance and control systems of the robot together with a report on the \emph{state quality} measure, which is used by the guidance and control module to adapt the mobility behavior of the system, ensuring safety and allowing recovery behaviors; for example, switching to velocity control when position estimates are bad or stopping the robot (or using attitude control in case of aerial vehicles) when velocity estimates are not reliable.

\ph{Modularity and SWaP}
The modular design of our estimation algorithm makes it very easy to leverage COTS (commercial-off-the-shelf) odometry solutions.
For example, one can easily combine any number of COTS LiDAR, thermal, and visual odometry algorithms to increase the resiliency of the system.
This modular design also allows for a selection of sensors and algorithms to accommodate for particular computational resources, power or payload, allowing to easily run minimal hardware and software architectures in real-time.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.75\linewidth]{figures/state_estimation/HeROdiagram}
  \caption{Schematics of HeRO: Heterogenous and Resilient Odometry estimation}
  \label{fig:hero}
\end{figure}

\begin{mybox}
\begin{center}
{\bf Capability: Robust and resilient state estimation}
\end{center}
State estimation architecture that allows redundancy in sensor and algorithmic modalities.
It considers failures as part of the design and enables self-recovery from malfunctioning.
The modularity of the design allows the use of self-designed or commercial-off-the-shelf solutions together with quick integration of new sensors and approaches.
\end{mybox}

\subsection{HeRO: Heterogenous and Resilient Odometry estimation}

\ph{Objective}
Our objective is to estimate the following robot states with respect to a ``world" frame along with their quality:\\
%\begin{tabular}{@{\hskip0pt}p{0.3\linewidth}@{\hskip1pt}p{0.7\linewidth}}
\begin{tabular}{cll}
&\hspace{1cm}$\vec{p} \in \mathbb{R}^3$ &\hspace{0.5cm}Position represented in world frame\\  
&\hspace{1cm}$\vec{R} \in SO(3)$ & \hspace{0.5cm}Orientation represented in world frame\\
&\hspace{1cm}$\vec{v} \in \mathbb{R}^3$ & \hspace{0.5cm}Linear velocity\\
&\hspace{1cm}$\vec{\omega} \in \mathbb{R}^3$ & \hspace{0.5cm}Angular velocity \\
&\hspace{1cm}$\vec{a} \in \mathbb{R}^3$ & \hspace{0.5cm}Linear acceleration\\
&\hspace{1cm}$\vec{\alpha} \in \mathbb{R}^3$ & \hspace{0.5cm}Angular acceleration\\
&\hspace{1cm}$Q_i \in \{Good, Bad\}$ & \hspace{0.5cm}Quality of $i$, with $i \in [\vec{p}, \vec{R}, \vec{v}, \vec{\omega}, \vec{a}, \vec{\alpha}]$
\end{tabular}\\
These states are used (when available) for motion planning and control, whereas the quality metrics are used by the behavior planner to select the appropriate mobility service for the current mission task.
Note that all attributes are represented in robot body frame unless stated otherwise. 
Moreover, we restricted the quality of the state to binary values although it can be easily generalized to higher resolutions and even continuous representations.
As previously mentioned, to obtain the best available estimation, HeRO consisting of the following main components:

\begin{enumerate}[label=\Alph*]
\item {\bf State estimation algorithms:}
Any single state estimation source can carry errors, either due to failures in sensor measurements, algorithms or both.
Hence, a part from selecting heterogeneous sensor modalities, we run in parallel a stack of heterogeneous odometry algorithms (\emph{e.g.}, visual, LiDAR, thermal, RaDAR or SoNAR), to increase the probability of overall success by having non-overlapping failure scenarios. 
There is no special requirement on the type of algorithm, with the ability to incorporate either tightly or loosely coupled approaches. 
However, to take advantage of all possible mobility services, there is a need for estimating position, orientation, velocity and, ideally, acceleration.
If the method is only estimating positions, it can be fused with IMU measurements (in a loosely coupled fashion) to obtain the rest of the state. 
This might be the case for pure visual or LiDAR odometry methods (VO and LO, respectively). Even though the software architecture of HeRO is tailored to incorporate a vast variety of estimation algorithms, we briefly describe hereafter the ones used in the DARPA Subterranean competition (Tunnel and Urban circuits).

\item {\bf Quality and health monitoring:}
The detection of malfunctioning odometry streams is a fundamental feature to select the best state estimation. 
Hence, it is of interest to define the possible failures in this context.
At a high level, a failure is any estimation that jeopardizes robot controls or planning.
Early identification of failures can allow for system recovery or, if recovery is not possible, performing safety fall-backs to keep the robot integrity.
HeRO detects the failures by running confidence checks at different levels of implementation.
First, HeRO performs confidence checks at hardware-level by checking the data from sensors. 
As an example, this type of checks in case of using cameras or LiDARs might include (but are not limited to): Rate of sensor output; overall image intensity or its variation within the image; distance between first and last return of a LiDAR beam; or number of invalid scan points.
% The selection of the best odometry stream will be based on identifying 
% Once we have multiple sources of odometry algorithms with disparate modes of failure, the next challenge is to identify those failures so that the optimal odometry source can be selected.
% Before continuing in further detail, the definition of failure in this context will be clarified. 
% At a high level, the goal is for reliable, high-rate state estimates for control/planning and failure is anything that jeopardizes that goal. 
% Early identification of the failures allows the system to perform actions to recover from failure or perform safety fall-backs to avoid hard collisions.
% To identify the type of failures as described in Table \ref{tab:xIO_summary}, HeRO first performs confidence checks at the hardware-level by using the data from sensors.
% The types of checks that are done here include:
% \begin{itemize}
%     \item Rate of sensor output. 
%     \item Overall image intensity or its variation within the image.
%     \item Distance between first and last return of a LiDAR beam.
%     \item Number of invalid scan points.
% \end{itemize}
%
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/state_estimation/failures.pdf}
    \caption{Different failure modes for odometry algorithms.}
    \label{fig:failure_modes}
\end{figure}
Next, HeRO performs confidence checks using data from the odometry algorithms, where the goal is to catch the failures depicted in Figure~\ref{fig:failure_modes}, ideally before they occur or at an early stage. 
These failures can come in a variety of forms, being a gap in the state updates, a divergence of the estimate, or rapid jumps. 
The failure could be caused by limitations of the sensor or by the overall odometry algorithm. 
The checks to detect these failures include: Rate of algorithm output (to catch gaps); rate of change of the position/velocity estimate (to catch jumps); and trace of the estimation covariance matrix (to catch divergence).
% \begin{itemize}
%     \item Rate of algorithm output (to catch gaps).
%     \item Rate of change of the position/velocity estimate (to catch jumps).
%     \item Trace of the estimation covariance matrix (to catch divergence).
% \end{itemize}
Notice how we can also run checks dependent on particularities of the methods; for instance number or quality of features tracked; or number or quality of inlier features (\emph{e.g.}, from matching/RANSAC).

\item {\bf Resiliency logic:}
The resiliency logic in HeRO is based on the outputs of the various odometry estimates and respective confidence checks, to output a resulting state estimate with its quality measure, which will be used by the planner and controller (\emph{i.e.}, depending on the state quality we can enable different mobility services).
Moreover, it supervises the individual odometry estimates and requires them to re-initialize in case of detecting failures.

An initial version of the logic can use a predefined ranking of odometry algorithms to select the best estimation method, thus selecting the approach with highest priority that is not failing. 
When that algorithm fails a confidence check, it is required to re-initialize while the next algorithm in the ranking is selected. 
These switches are provoked only in case of failure of the current source in order to minimizes the number of switches. 
A more advanced logic can consider a selection criteria weighted by the quality of the algorithm.
This comparison between streams also provides a third avenue for confidence checks; for instance, with three or more streams a voting scheme can be used to identify outliers.

The resiliency logic has to guarantee continuity in the resulting estimate while switching between streams. 
This consistency in the output can be achieved by iteratively composing an incremental state from the selected odometry source to the state from the previous estimate (\emph{e.g.}, a method estimating pose will re-start with its origin at {\bf 0}, hence if we switch to it after its re-initialization, we have to concatenate its estimation with the previous resulting state of HeRO).

% As described in the introduction, the architecture described here focuses on a loosely coupled, multiplexing approach, as opposed to a tightly coupled, fused approach. Nonetheless, a fusion of multiple algorithms and sensors can still be incorporated into this framework, as another odometry algorithm, or by fusing all state estimate streams that pass the confidence tests. 

% The resulting quality of the estimation is generated depending on the confidence checks in the odometry source being used. 
% Depending on this quality we can enable different mobility services, for instance position or velocity control (if position estimates are not available).
% , shown in Table~\ref{tab:state_quality} and detailed in the following section.
% % Note that ``medium" quality of a given odometry algorithm can occur on the failure of the front-end of a VIO (e.g. loss of feature tracking).  In this case, IMU measurements can be propagated to continue to get reliable velocity estimates for a short period even though position estimates may be bad. Velocity estimates alone are sufficient for control over such a period. 
% Note that in Table~\ref{tab:state_quality} we incorporated the platform height estimation ($^g{p}_z$) as a separate column because it can be directly used for the controller (altitude hold) and is an intermediate step between having all position estimates (${\bf p}$) or just velocities (${\bf v}$). Similarly, this sensor can be used to estimate vertical velocities ($v_z$). 
% These velocity-only states can appear either because they are directly provided by a method (\emph{e.g.}, optical flow) or because the logic decided to keep using an approach which is partially failing; for instance, using the output of a method that runs on IMU only while we reset the other update sources. 
% In the latter, velocities can be trusted for short periods.
% In Table~\ref{tab:state_quality}, we assume the IMU is not failing, providing good attitude (${\bf R}$), angular velocities (${\bm \omega}$) and accelerations (${\bf a}$,${\bm \alpha}$) with biases estimated by those methods previously working. 
% If that is not the case we consider an immediate landing in ``open loop" control mode.

% \begin{table}[t]
%     \centering
%     \begin{tabular}{|c|c|c|c|c|c|c|}
%     \hline
%     Case & \multicolumn{5}{c|}{State Quality} & Mobility \\
%     \hline
%     No. & ${\bf p}$ & $^{g}p_z$ & $v_x, v_y$ & $v_z$ & ${\bf R}$, ${\bm \omega}$, ${\bf a}$, ${\bm \alpha}$ & \\
%     \hline
%     1 & \cellcolor{green!25} & \cellcolor{green!25} & \cellcolor{green!25} 
%       & \cellcolor{green!25} & \cellcolor{green!25} & Global\\
%     \hline
%     2 & \cellcolor{red!25} & \cellcolor{green!25} & \cellcolor{green!25} 
%       & \cellcolor{green!25} & \cellcolor{green!25} & Local\\
%     \hline
%     3 & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{green!25} 
%       & \cellcolor{green!25} & \cellcolor{green!25} & Local\\
%     \hline
%     4 & \cellcolor{red!25} & \cellcolor{green!25} & \cellcolor{red!25} 
%       & \cellcolor{green!25} & \cellcolor{green!25} & Closed Loop on $z$\\
%     \hline    
%     5 & \cellcolor{red!25} & \cellcolor{red!25} & \cellcolor{red!25} 
%       & \cellcolor{red!25} & \cellcolor{green!25} & Attitude\\
%     \hline
%     \end{tabular}
%     \caption{Summary of available mobility services given different estimation qualities resulting from HeRO. The colour code is \colorbox{green!25}{Good} \colorbox{red!25}{Bad}.}
%     \label{tab:state_quality}
% \end{table}
\end{enumerate}

\subsection{Odometry algorithms}

We exploit two types of odometry estimation algorithms.
On the one hand we leverage existing estimation approaches (COTS).
This includes:
\begin{itemize}
    \item {\bf Wheel-Inertial}: For the wheeled platforms we can obtain an estimation of the 3D velocity vector $\vec{v}$ which can be fused with IMU measurements using, for instance, a traditional EKF. This wheel odometry information is available in most commercial wheeled platform as it is internally used by the platform controller.
    \item {\bf Kinematic-Inertial}: Similarly to the wheeled vehicles, the legged platforms compute internally the robot kinematics at a high rate for low-level control purposes. Particularly, we take advantage of SPOT platforms which already output these estimations.
    \item {\bf Visual-Inertial}: Visual inertial approaches have gained considerable attention in the last years, reaching a maturity that enables some of the existing solutions to be treated as COTS. This is the case of ORB-SLAM, a well known visual odometry estimation that can be directly fused with IMU measurements using a classic EKF.
\end{itemize}
On the other hand, the challenging conditions of the environments and the need for heterogeneity in our sensing suite required us to develop our own sensor fusion approach, in this case by means of LiDAR measurements. We fuse LiDAR measurements as follows.

\subsubsection{LiDAR-Inertial Odometry}

Unknown subterranean environments usually lack light, so the use of an active light sensor such as a LiDAR is very reasonable.
In most undergrounds situations, a LiDAR odometer solving for the motion between consecutive scans can produce fairly good trajectory estimates, however it lacks the sense of gravity. For this reason, in this work we exploit a pure LiDAR odometer and fuse its measurements with those from an IMU as shown in \autoref{fig:lio_architecture}. We divided our approach in two main modules, a \textit{front-end} computing pose estimates from LiDAR scans and pre-integrating IMU measurements; and a \textit{back-end} to fuse these observations. All related modules are briefly described hereafter.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.5\linewidth]{figures/state_estimation/lio_scheme.pdf}
  \caption{LiDAR-Inertial odometry architecture}
  \label{fig:lio_architecture}
\end{figure}

\underline{\bf LIO Front-end}

%Take from the paper Matteo is leading on Lidar Odometry - purely the front-end of the system. Summarise the approach and reference the paper. Add one example of results (better not to add a local map not to distract the reader), just a plot comparing with other odometries or error metrics, e.g. RMSE (root mean square error) of the method. Matteo probably has this in his paper already.

The \textit{front-end} of our LIO solution contains two main modules: a LiDAR odometer and IMU pre-integration.

\begin{itemize}[leftmargin=*]
    \item {\bf LiDAR-Odometry}
    %\textcolor{red}{TODO: Matteo, modify this section according to what LOCUS does. What is written now is the simpler front-end described in LION paper.} The LiDAR odometry module obtains relative pose measurements $ _{L_{k-1}}{\mathbf{T}}_{L_{k}}$ by using the Generalized Iterative Closest Point algorithm~\cite{segal2009generalized} on two LiDAR point clouds $P$ and $Q$ captured from consecutive LiDAR frames $L_{k}$ and $L_{k-1}$ at time stamps $k$ and $k-1$ respectively. To ease the convergence of the ICP algorithm, every incoming point cloud is pre-rotated in a gravity aligned-frame (i.e., setting the rotation estimated by the IMU as initial guess for ICP). 

\paragraph{Challenges and Limitations: }
Achieving consistent LiDAR odometry in perceptually-degraded environments is a challenging problem. The lack of reliable perceptual features in self-similar areas makes exteroceptive sensing ambiguous, and jerky sensor motion induced by navigation of harsh terrains poses significant threats to the on-board perception accuracy. In these settings, fusion of additional sensing modalities is therefore a vital step to achieve accurate operation under extreme perceptual conditions. While many multi-sensor LiDAR odometry methods that have been proposed can achieve great accuracy (~\cite{liosam2020shan}, ~\cite{ye2019tightly}, ~\cite{hess2016real}), they do not take into account potential failures of the fused sensing modalities (e.g. failure of VIO/IMU/LiDAR), which are likely to be observed in real-world field deployment, and that can result in catastrophic degradation of the odometry performance if not robustly handled. 

\paragraph{Proposed Solution: }
To overcome these challenges and enable reliable operation in extreme settings, we use LOCUS (LiDAR Odometry for Consistent operation in Uncertain Settings)~\cite{LOCUS}, a multi-sensor LiDAR-centric solution for high-precision odometry and 3D mapping in real-time. LOCUS provides a Generalized Iterative Closest Point (GICP)~\cite{segal2009generalized} based multi-stage scan matching unit equipped with an health-aware sensor integration module for seamless fusion of additional sensing modalities in a loosely coupled scheme. The proposed  solution is particularly suited to be deployed on robots navigating in extreme environments as \textit{(i)} it enables accurate and real-time operation under unfavorable sensing conditions and \textit{(ii)} is robust to intermittent and faulty measurements of the other fused sensing modalities.

\paragraph{System Description: }
Figure~\ref{fig:locus_architecture} reports the architecture of the proposed system, which is made of three main components: \textit{i)} point cloud preprocessor, \textit{ii)} scan matching unit, \textit{iii)} sensor integration module. The point cloud preprocessor is responsible for the management of multiple input LiDAR streams (e.g. syncing, motion-correction, merging, filtering) to produce a unified 3D data product that can be efficiently processed in the scan matching unit. The scan matching unit then performs a cascaded GICP-based scan-to-scan and scan-to-submap matching operation to estimate the 6-DOF motion of the robot between consecutive LiDAR acquisitions (the map is incrementally built by registering lidar acquisitions to the computed robot poses). In the pursuit of the joint optimization of accuracy and robustness, a key-component of the pipeline is the sensor integration module: in robots with multi-modal sensing, if available, we use an initial transform estimate from a non-lidar source to seed the GICP with a near-optimal prior in the  scan-to-scan matching stage, which improves accuracy and reduces computation, enhancing real-time performance. Multiple sources of odometry (e.g VIO,  KIO,  WIO) and raw IMU measurements available on-board are fed into a sensor integration module which selects the output from a priority queue of the inputs that are deemed healthy by a built-in health-monitor submodule. The priority order is based on the expected accuracy of the methods, such as: VIO, KIO, WIO, IMU, no input. The health metric currently used is simply the regular presence of the input messages, and can be extended to more sophisticated health monitoring paradigms, such as covariance checks. If the highest priority input is not healthy, then the next highest priority is used. 

\vspace{0.2cm}

\ph{Notation} 
We denote with $L_k$ the lidar acquisition collected at time $t_k$, and denote with $\textbf{E}^{k-1}_{k}$ the rigid body transformation of the sensor integration module output between two consecutive lidar acquisitions in the $[t_{k-1}, t_k]$ time interval, where $\textbf{E}^{k-1}_{k} \in SE(3)$. 

In the scan-to-scan matching stage (eq.~\ref{eq:GICP_scan_to_scan}), the GICP computes the optimal transformation $\hat{\textbf{T}}^{k-1}_{k}$ that minimizes the residual error $\mathcal{E}$ between corresponding points in $L_{k-1}$ and $L_{k}$. If the sensor integration module is successful, we initialize the GICP with $\textbf{T}^{k-1}_{k} = \textbf{E}^{k-1}_{k}$. If all sensors fail, the GICP is initialized with identity pose and the system reverts to pure lidar odometry.

\begin{align}
\label{eq:GICP_scan_to_scan} \hat{\textbf{T}}^{k-1}_{k} = \arg\min_{\textbf{T}^{k-1}_{k}} \mathcal{E} (\textbf{T}^{k-1}_{k}L_{k}, L_{k-1})
\end{align}



The motion estimate produced by the scan-to-scan matching stage is further refined by a scan-to-submap matching step (eq.~\ref{eq:GICP_scan_to_submap}), where the current lidar acquisition is matched against a robot-centered submap $S_k$. In this optimization, $\textbf{T}^{k-1}_{k}$ is initialized with the $\hat{\textbf{T}}^{k-1}_{k}$ result from eq.~\ref{eq:GICP_scan_to_scan}.

\begin{align}
\label{eq:GICP_scan_to_submap} \hat{\textbf{T}}^{k-1}_{k} = \arg\min_{\textbf{T}^{k-1}_{k}} \mathcal{E} (\textbf{T}^{k-1}_{k}L_{k}, S_{k})
\end{align}

\paragraph{Evaluation against state-of-the-art: }
We compare LOCUS against state-of-the-art, open source, LiDAR odometry methods (~\cite{liosam2020shan}, ~\cite{ye2019tightly},~\cite{hess2016real},~\cite{LOAM}, ~\cite{BLAM}) in extreme, perceptually-degraded subterranean environments, and demonstrate top-class localization accuracy, along with substantial improvements in robustness to sensor failures. For the evaluation,  we  use  the  data  collected  in  the Tunnel and Urban Circuit rounds of the DARPA Subterranean Challenge, from  a  wheeled  ground  robot carrying two LiDAR sensors, an IMU and running WIO onboard. The environments of interest are a test-mine in Pittsburgh, PA, and a dismissed power plant located in Elma, WA, that present many challenges for robot perception such as long feature-poor corridors and big open spaces. 

In the accuracy evaluation, we compute the absolute position error (APE) of the estimated robot trajectory against the ground-truth reference, for the different methods over the different runs, and report in \autoref{fig:locus_architecture} a summary of the results. LOCUS achieves top-class localization accuracy, ranking 1st in the Alpha and Beta courses of the Urban Circuit and 3rd in the Safety Research course of the Tunnel Circuit.

In the robustness evaluation, we analyze the robustness and flexibility of the various methods with respect to sudden failure of an input source by testing the following failure scenarios: (\emph{i) failure of WIO/IMU;  (\emph{ii}) failure of WIO; and, (\emph{iii}))} failure of LiDAR; and report in \autoref{fig:locus_robustness} a summary of the results with the map produced by the different algorithms in the Beta course dataset. 

In the first test (\autoref{fig:locus_robustness} (a)) we simulate a shut-down of the WIO stream after 1200s, while in the second test (\autoref{fig:locus_robustness} (b)), we simulate a simultaneous shut down of WIO and IMU streams after 1200s. Tightly-coupled approaches, as well as methods designed with synced callbacks, stop operating when a input is missing. In contrast, LOCUS automatically engages its recovery behaviour, switching from LiDAR odometry with WIO integration to LiDAR odometry with IMU integration in the first case, and from LiDAR odometry with WIO integration to LiDAR odometry with IMU integration to pure LiDAR odometry in the second case, continuing its journey. 

In the third test (\autoref{fig:locus_robustness} (c)), we simulate a 10 s gap in LiDAR feed while the robot is in motion, between 1200s and 1210s. This failure mode challenges all methods, resulting in evident degradation of the LiDAR registration accuracy around the failure location. LOCUS instead leverages the accumulation of WIO over the period where the LiDAR is not present, to produce an accurate initial transform when the LiDAR returns, resulting in consistent ego-motion estimation and mapping.

Overall, LOCUS consistently exhibits the greatest robustness, demonstrating efficient handling of sensor failures in a cascaded fashion, behaviour that is highly desirable to accommodate the unforeseen challenges posed by real-world operations where hardware failures are likely to happen, or sensor sources can become unreliable (e.g. dark areas with no visual texture for VIO).

\begin{figure}[t]
  \centering
  \includegraphics[width=0.5\linewidth]{figures/state_estimation/locus_architecture.pdf}
  \caption{LOCUS architecture}
  \label{fig:locus_architecture}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.95\linewidth]{figures/state_estimation/locus_accuracy.pdf}
  \caption{LOCUS accuracy}
  \label{fig:locus_architecture}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.55\linewidth]{figures/state_estimation/locus_robustness.pdf}
  \caption{LOCUS robustness}
  \label{fig:locus_robustness}
\end{figure}

\item {\bf IMU pre-integration}
    
The IMU pre-integration module leverages the state-of-the-art on-manifold pre-integration theory to summarize the high-rate IMU measurements into a single motion constraint~\cite{forster2015imu} \cite{forster2015manifold} for the subsequent pose-graph optimization performed in the back-end of the algorithms. IMU pre-integration is also used to guarantee a pose and velocity estimate, output of the algorithms, at high-rate, regardless of the time taken by the optimizer.
\end{itemize}

\underline{\bf Back-end}

\textbf{Description of State, Measurements and Output} The fusion of the relative pose-measurement obtained from LiDAR odometry and from IMU pre-integration is performed via a fixed-lag smoother, using a factor graph to store the output of the front-end. More details about the approach and the fusion scheme can be found in our related work \cite{LION}. More specifically, the proposed back-end is employed to estimates the pose (position and attitude) and velocity of a single robot. The algorithm does not require any calibration phase, as the extrinsic calibration between the LiDAR and the IMU, as well as the IMU biases, are estimated on-line.  Poses are estimated with respect to an inertial (but potentially slowly drifting) odometry reference frame $W$, and a body reference frame $B$, attached to the center of the IMU. We additionally assume the LiDAR frame $L$ to be attached to the center of the LiDAR. 
The state vector  $\mathbf{{x}}_{j}$  of the estimator at the $j$-th time step is thus given by:
\begin{equation}
    \mathbf{{x}}_{j}:=\{\:_{W}\mathbf{T}_{B},\:_{W}\mathbf{v}
    ,\:_{B}\mathbf{b}^{a},\:_{B}\mathbf{b}^{g},\:_{B}\mathbf{T}_{L}\}_{j}\,
\end{equation}
where $\:_{W}\mathbf{T}_{B}$ is the IMU-to-world transformation, $_W \mathbf{v}$ is the linear velocity, $_B \mathbf{b}^a$ and $_B \mathbf{b}^g$ are the accelerometer and gyroscope biases of the IMU, and $\:_{B}\mathbf{T}_{L}$ is the lidar-to-IMU transformation. A representation of the states and factors used in the factor graph with a window of $k$ time steps can be found in \autoref{fig:factor_graph_colored}. 
The measurements are provided by the two front end units and are added synchronously to the factor graph.
To reduce the effects of error in mounting the sensors, the back-end can actively estimated the extrinsic calibration (translation and rotation) between the LiDAR and the IMU. These parameters are estimated via the calibration factor, which is added in between every pose values, as shown in \autoref{fig:factor_graph_colored}. For computational efficiency, the factor is added to the graph at a lower rate than i.e. the relative pose measurements. 
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/state_estimation/factor_graph_colored.pdf}
    \caption{Factor graph representing state and measurements used by the back-end. In this figure we use the shortcut $\boldsymbol{b}_j:=\{\mathbf{b}^{a}, _{B}\mathbf{b}^{g}\}_j$ for the biases. Here  for visualization purposes, we illustrate the initialization of the optimization (with the prior factors).
    }
    \label{fig:factor_graph_colored}
\end{figure}

\textbf{Solving the Optimization Problem}
Given the relative-pose and IMU measurements $\mathcal{{Z}}_{k}$ stored in the factor-graph, following \cite{forster2015manifold}, we perform smoothing within the sliding window by minimizing the negative log-likelihood of the posterior distribution $p\left(\mathcal{X}_{k}|\mathcal{Z}_{k}\right)$, where $\mathcal{X}_{k}$ are the state-variables in the window. 
We model the optimization problem using GTSAM \cite{dellaert2012factor} and solve this optimization problem using iSAM2 \cite{kaess2012isam2}.
%The measurements are provided by the two front end units and are added synchronously to the factor graph.
%To reduce the effects of error in mounting the sensors, the back-end can actively estimated the extrinsic calibration (translation and rotation) between the LiDAR and the IMU. These parameters are estimated via the calibration factor, which is added in between every pose values, as shown in Fig. \ref{fig:factor_graph_colored}. For computational efficiency, the factor is added to the graph at a lower rate than i.e. the relative pose measurements. 

\textbf{Evaluation Setup} We evaluate the performance of the back-end in the sensor data recorded in the Tunnel Competition, held in the NIOSH experimental mines in Pittsburgh, USA. 
To showcase the performance of our fusion approach, in this evaluation we use as LiDAR-odometry input the more challenging (due to large drifts) Scant-To-Scan odometry, which corresponds the raw relative pose estimates obtained from ICP between two consecutive single-LiDAR measurements. Scant-To-Scan odometry measurements are fused at 10 Hz, while IMU and back-end output could be provided at up to 200 Hz. The length of the sliding window is 6 seconds.
For reference, we compare the performance of our approach to Wheel-Inertial odometry and Scan-To-Scan odometry (the relative pose input of the back-end), with LAMP~\cite{LAMP} as ground truth. A more in depth analysis of the results across multiple days of competition is provided in \cite{LION}. 

\textbf{Evaluation Results} The results for a $676$ m - long, $1520$ s run are summarized in \autoref{fig:day1_h1_position_error} and \autoref{fig:day1_h1_attitude_error}. We can observe that fusing inertial data with the odometry obtained from Scan-To-Scan ICP significantly reduces the drift of the pure LiDAR-odometry method (Scan-To-Scan). This is especially evident from the estimation error along the $z$-axis shown in \autoref{fig:day1_h1_position_error}. Additionally, the proposed back-end reliably estimates the attitude of the robot (\autoref{fig:day1_h1_attitude_error}), achieving small roll and pitch errors (since they are observable in the IMU via the gravity vector) and yaw. \autoref{fig:day1_h1_XYZ} shows that the proposed back-end outperforms the baseline approach (Wheel-Inertial) especially in terms of drift in yaw and horizontal translation. To showcase the auto-calibration capabilities, we generate in simulation a dataset where the LiDAR is translated of $0.1$ m with respect to the IMU, along the IMU's $y$-axis. In \autoref{fig:auto_calibration_error} we observe that after approximately $20$ s, our approach (continuous lines) estimates the correct extrinsics (dotted lines). 
\begin{figure}
  \centering
  \begin{minipage}[b]{0.48\textwidth}
    \includegraphics[trim=0 250 70 120,clip,width=\textwidth]{figures/state_estimation/day1_h1_position_error_RMSE.pdf}
    \caption{Position estimation RMSE.}
    \label{fig:day1_h1_position_error}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.48\textwidth}
    \includegraphics[trim=0 250 70 120, clip,width=\textwidth]{figures/state_estimation/day1_h1_attitude_error_RMSE.pdf}
    \caption{Attitude estimation RMSE.}
    \label{fig:day1_h1_attitude_error}
  \end{minipage}
  \centering
  \begin{minipage}[b]{0.48\textwidth}
    \includegraphics[trim=20 245 30 120,clip,width=\textwidth]{figures/state_estimation/day1_h1_XY_600s_run2.pdf}
    \caption{Qualitative evaluation of the $xy$ position estimates for the first 600s of the considered run.}
    \label{fig:day1_h1_XYZ}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.48\textwidth}
    \includegraphics[trim=0 0 0 0, clip, width=\textwidth]{figures/state_estimation/auto-calibration-v6.png}
    \caption{Estimation of the translation of the extrinsics.}
    \label{fig:auto_calibration_error}
  \end{minipage}
\end{figure}
 





%\hspace{2em}{\bf LiDAR and IMU fusion: LION and LIO-EKF}

\begin{mybox}
{\centering {\bf Current status}}

The robust and resilient state estimation capability has been fully developed in its initial version, and the validation and utility of the module has demonstrated high performance in real experiments using different types of robots and in the DARPA Subterranean Challenge, Tunnel and Urban circuits.

{\bf Future work}

The current state estimation architecture considers a loosely coupled approach, with several odometry estimation methods and a resiliency logic that supervises health of estimations and multiplexes between the best of them, depending on availability (HeRO).
This architecture offers several advantages as described above, however, in the near future we are pushing for an actual fusion of the odometry estimations and incorporate a robust outlier rejection layer.

\end{mybox}

==> template_files/instructions.tex <==
\section*{\comb{ {\bf @CoSTARs}: Please have a look at the following formatting instructions}}
\comb{
\subsection{General formatting instructions}
\label{gen_inst}

The main text of your paper should be in a single column textbox 6.5
inches by 9 inches. Regular text should be in a 12 point font.
Paragraphs should not be indented, and should be separated by a
single line space.

Please pay attention to the instructions in the next section 
regarding figures, tables, acknowledgments, and references.

\subsubsection{Formulation}

I've added the mathsym.tex file to standardize the addition of formulas. I suggest to use the following:
\begin{equation}
\begin{split}
    \bfM: Matrix \\
    \bfv: Vector \\
    s: Scalar    
\end{split}
\end{equation}

Please, when adding your stuff, try to follow some standards so it'll be easier later on.

\subsubsection{Citations within the text}

Citations should follow the APA style \cite{apa}. Unlike many
scientific papers, this requires in text citation of authors' names
and date of work. The corresponding references are to be listed in
alphabetical order using APA reference style at the end of the
paper, in the \textbf{References} section. Example references are
given in this template for books with one author \cite{baxter},
conference papers \cite{binh}, journal articles \cite{baldwin}, and
books with editors \cite{stock}. For electronic references without
authors, the reference is cited using the web page title. The
University of Wisconsin Writing Center provides a good resource for
questions about the APA style \cite{wisconsin}.

\subsubsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first
footnote} in the text. Place the footnotes at the bottom of the page
on which they appear. Precede the footnote with a horizontal rule of
2~inches.\footnote{Sample of the second footnote}

\subsubsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. We recommend using either the jpg or the embedded
postscript format for images and the tiff format for line drawings.
If the figures contain graphs, please ensure that the axis labels
are legible when printed. Figure number and caption always appear
after the figure. Place one line space before the figure caption,
and one line space after the figure. The figure caption is lower
case (except for first word and proper nouns); figures are numbered
consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

\begin{figure} [h]
    \centering
    \includegraphics[height=2.0in]{figures/g1}
    \hspace{.2in}
    \includegraphics[height=2.0in]{figures/g2}
    \caption{Line graph of random numbers (left) and bar graph of random numbers (right)}
    \label{fig:sampleFigure}
\end{figure}

\subsubsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. Table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title} \label{sample-table}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|}
  \hline
% after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
   & $k_{g}$ & $k_{o}$ & $c_{3}$ & $c_{4}$ & $c_{5}$ \\
  \hline\hline
  Careful/Sparse & 0.334 & 0.597 & 1.101 & 9.621 & 8.170 \\ \hline
  Careful/Dense & 3.124 & 3.195 & 1.094 & 5.899 & 7.318 \\ \hline
  Aggressive/Sparse & 0.840 & 9.153 & 2.853 & 8.274 & 0.187 \\ \hline
  Aggressive/Dense & 4.838 & 2.841 & 0.670 & 7.952 & 0.386 \\ \hline
  Hand-Tuned & 0.767 & 0.060 & 0.340 & 2.000 & 0.250 \\
  \hline
\end{tabular}
\end{center}
\end{table}

\subsubsection{APA Reference Style}

References follow the acknowledgments. Use an unnumbered third level
heading for the references. References must be listed in the APA
format (available at http://www.apastyle.org/). References should be
in the same font size as the paper text.


} % end of comb
